Query matching for spatio-temporal action detection with query-based object detector

In this paper, we propose a method that extends the query-based object detection model, DETR, to spatio-temporal action detection, which requires maintaining temporal consistency in videos. Our proposed method applies DETR to each frame and uses feature shift to incorporate temporal information. However, DETR's object queries in each frame may correspond to different objects, making a simple feature shift ineffective. To overcome this issue, we propose query matching across different frames, ensuring that queries for the same object are matched and used for the feature shift. Experimental results show that performance on the JHMDB21 dataset improves significantly when query features are shifted using the proposed query matching.

==> settings.tex <==
\usepackage{graphicx}
\usepackage[sort,space,adjust,compress]{cite}


\usepackage[pagebackref=true,breaklinks=true,colorlinks,bookmarks=false,dvipdfmx]{hyperref}
\usepackage{amsmath}
\usepackage{amssymb}


\usepackage{multirow}
\usepackage{multicol}
\usepackage{diagbox}
% \usepackage{slashbox}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[labelformat=simple]{subcaption}
\renewcommand\thesubfigure{(\alph{subfigure})}% Fig\ref{fig:label} --> Fig.8(a)
\renewcommand\thesubtable{(\alph{subtable})}% Tab\ref{tab:label} --> Tab.8(a)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{algorithmic}
\usepackage{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

% \makeatletter
% \renewcommand{\ALG@name}{アルゴリズム}% only for Japanese
% \makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{caption}
\captionsetup{labelsep=colon}% figure, table
\captionsetup[ruled]{labelsep=colon}% algorithm



\addtolength{\oddsidemargin}{0mm}
\addtolength{\evensidemargin}{0mm}

\renewcommand{\topfraction}{0.9}
\setcounter{topnumber}{3}



%%%%%%%%%%%%%%%%%%%%%%%% examples for equations
\newcommand{\R}{\mathbb{R}}

\newcommand{\x}{\boldsymbol{x}}
\newcommand{\y}{\boldsymbol{y}}
\newcommand{\X}{\boldsymbol{X}}

\newcommand{\T}{\mathcal{T}}

\newcommand{\similarlity}{\mathrm{sim}}

\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
%%%%%%%%%%%%%%%%%%%%%%%%

